SuperNeurons: Dynamic GPU Memory Management for Training Deep Neural Networks

Going deeper and wider in neural architectures improves the accuracy, while the limited GPU DRAM places an undesired restriction on the network design domain. Deep Learning (DL) practitioners either need change to less desired network architectures, or nontrivially dissect a network across multiGPUs. These distract DL practitioners from concentrating on their original machine learning tasks. We present SuperNeurons: a dynamic GPU memory scheduling runtime to enable the network training far beyond the GPU DRAM capacity. SuperNeurons features 3 memory optimizations, \textit{Liveness Analysis}, \textit{Unified Tensor Pool}, and \textit{Cost-Aware Recomputation}, all together they effectively reduce the network-wide peak memory usage down to the maximal memory usage among layers. We also address the performance issues in those memory saving techniques. Given the limited GPU DRAM, SuperNeurons not only provisions the necessary memory for the training, but also dynamically allocates the memory for convolution workspaces to achieve the high performance. Evaluations against Caffe, Torch, MXNet and TensorFlow have demonstrated that SuperNeurons trains at least 3.2432 deeper network than current ones with the leading performance. Particularly, SuperNeurons can train ResNet2500 that has $10^4$ basic network layers on a 12GB K40c.

==> rebuttal_tim <==
Dear Reviewers:

We thank the reviewers for the very helpful feedback on our paper. 

===========Reviewer 46A

\textbf{46A-1}-How are the challenges of non-linear DNN different from normal DNN in terms of the 
pressure on GPU memory and will the proposed approach works for linear DNN as well?

That is a very good observation. In fact, the same techniques can be used for linear DNN 
and should also help. However, we note that the best linear network on ImageNet is VGG-19 
having 25 sequentially connected layers. In contrast, the best non-linear models are much 
deeper (e.g., ResNet-50 has 152 layers and ResNet-152 has 458 layers). Thus we focussed on 
non-linear models mainly because of their size and the importance of good memory management 
for them. We will clarify this in the paper and if space permits, also include numbers for 
at least one linear model.

%%46A-2-It will be good if the authors can show the performance breakdown in Table 2.

This is an excellent suggestions which we will address in the final version. 
For AlexNet, the breakdown looks as follows:
a) the effect of Tensor Cache w.r.t on-demand prefetch/offloading toward the speed:
AlexNet—batch:128—with LRU: 433 img/s—On-demand Prefetch/Offloading:367 img/s
b)the effect of dynamic workspace allocations w.r.t static convolution workspace allocations 
toward the speed:
AlexNet—batch:128—dynamic:421 img/s—static:390 img/s

%%46A-3-What are the performance [breakdowns] compared to others such as TensorFlow?
Unfortunately, it is very hard to get a performance breakdown for other systems like TensorFlow. 
Therefore we only did an end-to-end evaluation against other deep learning frameworks as shown 
in Figure 14. 

%%46A-4-The mathematical parameters are not defined in the paper
We defined them in Section 3, however, for the final version we will clarify that in introducing 
the notation earlier on. 

%%46A-5-For unified tensor pool, how the runtime figure out which data/tensor should be offloaded/prefetched? 

The idea behind the Tensor Cache is relatively simple: we try to cache as many tensors as 
possible on the GPU memory and if not enough memory is available, we offload the tensors 
to main memory based on LRU. All current required tensors are pinned to the GPU 
(i.e., there can not be removed based on LRU). We always try to prefetch X-steps (usually 5), 
prefetched in order using the following procedure: .1) Offload as many tensors with lowest 
LRU score to main memory, which are not pinned. 2.1) If enough space exist, prefetch the 
tensors for the next step and pin them (so that they can not be removed) 2.2) If not enough 
space exist, fail this and all following prefetch operations. This procedure continues with 
after the completion of every step. 

We will clarify this procedure for the final camera ready.

%%46A-6-Since it focuses on non-linear DNNs, will LRU a good policy for offloading? 
What are the hit rate of the "tensor cache"?

While we acknowledge that LRU not necessarily will provide the optimal memory allocation, 
we found it extremely practical. For example, for prefetching many tensors are already in 
the cache and simply need to be pinned. We also measured the hit rate for some of our networks. 
For example, for ResNet152: batch:48 the hit rates is 98.02% (hit=5536, miss=112). With a 
batch size of 96, the hit rate is 91.22% (hit=5152, miss=496). Studying other cache-policies 
are ways to better utilize the fact, that we know the dependency graph from the network 
configuration, are beyond the scope of this paper.

===========Reviewer 46B

%%46B-1-contrast Chen’s arXiv paper with your approach?

We actually did cite it (it is reference [6]) and it was one of the papers, which strongly 
motivated cost aware re-computation. However, we are able to achieve more memory savings as 
we have a more fine grained approach as seen in Table 1 (the fastest approach is the one 
from reference [6]). Also as our experiments in Figure 11 show, this can have a real impact 
on what model size one is able to run on the GPU.

We will clarify our comparison to [6] in more detail when we prepare the camera ready and 
also make it explicit in Table 1 and Figure 11, that we compare against [6]. 
 
%%46B-2-How do you come to the conclusion of "optimal" training speed? 

That was an oversight on our side. Obviously, it should not be called optimal and we already 
know, that we create better caching policies. We will correct this mistake in the next iteration 
of the paper and also - by means of an example - show when our LRU strategy is in fact not optimal.

%%46B-3-There were several places were I would have liked to have seen more detail about 
how the system achieves its claims.

Thanks for the comment. Please see also our answer to 46A-5 where we describe the general 
caching procedures. We will improve the descriptions by modeling operations into primitives
such as LRU and Tensor Allocations. We will present a global procedure
to elucidate internal cooperations among different primitives in the final draft. 

%%46B-4-DenseNet experiments
Thank you, we will include experiments on DenseNet in the final draft.

%%46B-5-Why did you use a K40 and not something newer like a Titan X (either Pascal or Volta)?
At the time, we only had access to K40c. Tensor core is recently introduced in Volta, 
but we do have Pascal now. The degree of overlapping only affects the speed; and the speed 
trend on Titan-Xp is similar to K40c. We will provide evaluations on TITAN-Xp in Fig.14.

%%46B-6-more narrow range of batch sizes but with a wider array of deep neural networks 
since that is your stated goal.

Great suggestions. The reported deepest ResNet on ImageNet is ResNet152, while the deepest 
ResNet trained by our framework is ResNet2500 (10000 basic layers), nearly 20x deeper than 
state-of-the-art. The batch size of ResNet2500 is 1 to get the deepest model. We will add 
inception v4 and DenseNet with a focus on small batches in the final draft.

===========Reviewer 46C

%%46C-1-The claims that memory usage and training speed are optimal are not justified.

Claiming speed optimality is indeed an oversight on our side, and we will address it.

We claim the memory optimality under the assumption of layer-wise computations implemented 
in cuDNN. That's being said, a layer's memory usage in any networks must less than GPU onboard 
memory. Therefore, the largest computable network is the one with max(l_i) = GPU RAM,
where l_i is the memory usage of a layer. In Fig.11, we demonstrate that 3 memory optimization
techniques successfully reduce the peak memory usage to max(l_i). Therefore, we claim achieving
the memory optimality.

%%46C-2-Figure 2

Thank you for suggestions, and we will change the unit of left axis to GB. We will separate 
two graphs in Fig.2 to clarify it. The left y-axis of Fig.2 (Memory allocations in MB) is 
for the bar plot explaining the actually memory usages, while the right y-axis  
(speedups with convolution buffer) is for the red line.

%%46C-3-Equation Definition
Thank you. We defined the memory notations in Section 3, and we will clarify them ahead in
the final draft.

%%46C-4-the unified memory pool should be described with some primitives rather than some 
fairly vague text.

Thanks for the comment. Please kindly see our answer to 46A-5 where we present the general 
caching procedure. We will elucidate the unified memory pool with primitives such as LRU 
and Tensor Allocations in the final version.
